Cross-Resolution Adversarial Dual Network for Person Re-Identification and Beyond

Person re-identification (re-ID) aims at matching images of the same person across camera views. Due to varying distances between cameras and persons of interest, resolution mismatch can be expected, which would degrade re-ID performance in real-world scenarios. To overcome this problem, we propose a novel generative adversarial network to address cross-resolution person re-ID, allowing query images with varying resolutions. By advancing adversarial learning techniques, our proposed model learns resolution-invariant image representations while being able to recover the missing details in low-resolution input images. The resulting features can be jointly applied for improving re-ID performance due to preserving resolution invariance and recovering re-ID oriented discriminative details. Extensive experimental results on five standard person re-ID benchmarks confirm the effectiveness of our method and the superiority over the state-of-the-art approaches, especially when the input resolutions are not seen during training. Furthermore, the experimental results on two vehicle re-ID benchmarks also confirm the generalization of our model on cross-resolution visual tasks. The extensions of semi-supervised settings further support the use of our proposed approach to real-world scenarios and applications.

==> exp/dataset.tex <==
\begin{table}[t]
  \small
  \ra{1.3}
  \begin{center}
  \caption{Statistics of the adopted datasets.}
  %
  \vspace{\tablecapmargin}
  \label{table:dataset-stat}
  \resizebox{1\linewidth}{!} 
  {
  \begin{tabular}{l|ccc|c}
  %
  \toprule
  %
  \multirow{2}{*}{Dataset} & \multicolumn{3}{c|}{Statistics} & \multirow{2}{*}{Down-sampling} \\
  %
   & \# of images & \#  of cameras & \# of identities &\\
  %
  \midrule
  %
  MLR-CUHK03 & 14000 & 5 & 1467 & \checkmark ($r \in \{2, 3, 4\}$) \\
  %
  MLR-ViPeR & 1264 & 2 & 632 & \checkmark ($r \in \{2, 3, 4\}$) \\
  %
  CAVIAR & 1220 & 2 & 72 & \xmark \\
  %
  MLR-Market-1501 & 32668 & 6 & 1501 & \checkmark ($r \in \{2, 3, 4\}$) \\
  %
  MLR-DukeMTMC-reID & 36411 & 8 & 1404 & \checkmark ($r \in \{2, 3, 4\}$) \\
  %
  \midrule
  %
  Market-1501 & 32668 & 6 & 1501 & \xmark \\
  %
  DukeMTMC-reID & 36411 & 8 & 1404 & \xmark \\
  %
  \bottomrule
  %
  \end{tabular}
  }
  \end{center}
  \vspace{-2.0mm}
\end{table}

==> exp/exp-LR.tex <==
%
\begin{table}[h]
  \small
  \ra{1.3}
  \begin{center}
  \caption{Train multi-scale LR images and test on lowest resolution images.}
  %\vspace{\tablecapmargin}
  \label{table:exp-LR}
  \resizebox{\linewidth}{!} 
  {
  \begin{tabular}{l|l|l|ccccc}
  %
  \toprule
  %
  \multirow{2}{*}{Train} & \multirow{2}{*}{Test} & \multirow{2}{*}{Method} & \multicolumn{5}{c}{CUHK03} \\
  %
  & & & Rank 1 & Rank 5 & Rank 10 & Rank 20 & mAP \\
  %
  \midrule
  %
  \multirow{2}{*}{D=4} & \multirow{2}{*}{D=4} & Ours (single-level) & 71.3 & 94.1 & 97.9 & 99.4 & 66.9 \\
  %
  & & Ours (single-level RK) & 83.2 & 96.3 & 98.6 & 99.5 & 80.7 \\
  %
  \midrule
  %
  \multirow{2}{*}{D=2,3,4} & \multirow{2}{*}{D=4} & Ours (single-level) & 73.0 & 94.7 & 98.0 & 99.3 & 69.8 \\
  %
  & & Ours (single-level RK) & 81.3 & 96.0 & 98.3 & 99.4 & 79.1 \\
  %
  \midrule
  %
  \multirow{2}{*}{D=8} & \multirow{2}{*}{D=8} & Ours (single-level) & 55.6 & 86.1 & 92.8 & 97.3 & 51.0 \\
  %
  & & Ours (single-level RK) & 66.7 & 89.3 & 93.9 & 97.5 & 63.2 \\
  %
  \midrule
  %
  \multirow{2}{*}{D=2,4,8} & \multirow{2}{*}{D=8} & Ours (single-level) & 62.7 & 90.7 & 96.2 & 98.8 & 58.5 \\
  %
  & & Ours (single-level RK) & 73.6 & 92.7 & 96.7 & 98.9 & 70.4 \\
  %
  \bottomrule
  %
  \end{tabular}
  }
  \end{center}
  \vspace{\tablemargin}
\end{table}

==> exp/exp-multi-Re.tex <==
\begin{table}[t]
  \small
  \ra{1.3}
  \begin{center}
  \caption{Effect of training images of multiple low resolutions. The bold numbers indicate the best results.}
  \vspace{\tablecapmargin}
  \label{table:exp-multi-resolution}
  \resizebox{\linewidth}{!} 
  {
  \begin{tabular}{ll|cc|cc|cc}
  %
  \toprule
  %
  \multicolumn{2}{l|}{Train} & \multicolumn{2}{c|}{MLR-CUHK03} & \multicolumn{2}{c|}{MLR-VIPeR} & \multicolumn{2}{c}{CAVIAR} \\
  %
  HR & LR & Rank 1 & mAP & Rank 1 & mAP & Rank 1 & mAP \\
  %
  \midrule
  %
  $r = 1$ & $r = 2$ & 70.9 & 67.7 & 38.9 & 42.6 & 36.3 & 52.9\\
  %
  $r = 1$ & $r = 3$ & 72.3 & 68.8 & 40.3 & 43.2 & 37.9 & 53.1\\
  %
  $r = 1$ & $r = 4$ & 77.2 &74.8 & 41.5 & 45.4 & 40.1 & 54.6\\
  %
  $r = 1$ & $r \in \{2, 3, 4\}$ & \textbf{78.9} & \textbf{75.9} & \textbf{42.5}& \textbf{47.0}& \textbf{42.0}& \textbf{56.3}\\
  %
  \bottomrule
  %
  \end{tabular}
  }
  \end{center}
  \vspace{2.0\tablemargin}
\end{table}

==> exp/visual_intro.tex <==
\setlength{\fiveimg}{0.1\linewidth}
\begin{figure*}[t]
  \ra{1.3}
  \centering
  \begin{subfigure}[b]{\dimexpr\fiveimg+12pt\relax}
    \makebox[6pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\scriptsize Baseline }}}%
    \makebox[6pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\scriptsize (Train on HR)}}}%
    \includegraphics[width=0.95\fiveimg,cfbox=white 1pt 1pt]{rank-sample/Q_8.png}\\
    \makebox[6pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\scriptsize Baseline (Train}}}%
    \makebox[6pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\scriptsize on HR \& LR)}}}%
    \includegraphics[width=0.95\fiveimg,cfbox=white 1pt 1pt]{rank-sample/Q_8.png}\\
    \makebox[12pt]{\raisebox{20pt}{\rotatebox[origin=c]{90}{\scriptsize Ours}}}%
    \includegraphics[width=0.95\fiveimg,cfbox=white 1pt 1pt]{rank-sample/Q_8.png}\\
    \vspace{\figmargin}
    \caption*{\hspace{5mm}\scriptsize Query}
  \end{subfigure}
  %
  \hskip .1em
  \vrule
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/403.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/557.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/407.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 1}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/408.png}\\ 
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/408.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/402.png}\\
    \vspace{\figmargin} 
    \caption*{\scriptsize Top 2}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/703.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/403.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/411.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 3}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/402.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/411.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/404.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 4}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/549.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/406.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/409.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 5}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/564.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/402.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/406.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 6}
  \end{subfigure}
  %
  \hskip .2em
  %
  \begin{subfigure}[b]{\fiveimg}
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/700.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=red 1pt 1pt]{rank-sample/565.png}\\
    \includegraphics[width=0.95\linewidth,cfbox=green 1pt 1pt]{rank-sample/408.png}\\
    \vspace{\figmargin}
    \caption*{\scriptsize Top 7}
  \end{subfigure}
  %
  \caption{Example of the top-ranked HR gallery images of the MLR-CUHK03 dataset which are matched by the LR query input. Images bounded in green and red rectangles denote correct and incorrect matches, respectively.}
  %
  \vspace{0.8\figmargin}
  \label{fig:rank}
\end{figure*}


